Do You See What I See? Coordinating Multiple Aerial Cameras for Robot Cinematography

Aerial cinematography is significantly expanding the capabilities of film-makers. Recent progress in autonomous unmanned aerial vehicles (UAVs) has further increased the potential impact of aerial cameras, with systems that can safely track actors in unstructured cluttered environments. Professional productions, however, require the use of multiple cameras simultaneously to record different viewpoints of the same scene, which are edited into the final footage either in real time or in post-production. Such extreme motion coordination is particularly hard for unscripted action scenes, which are a common use case of aerial cameras. In this work we develop a real-time multi-UAV coordination system that is capable of recording dynamic targets while maximizing shot diversity and avoiding collisions and mutual visibility between cameras. We validate our approach in multiple cluttered environments of a photo-realistic simulator, and deploy the system using two UAVs in real-world experiments. We show that our coordination scheme has low computational cost and takes only 1.17 ms on average to plan for a team of 3 UAVs over a 10 s time horizon. Supplementary video: https://youtu.be/m2R3anv2ADE

==> inputs/3_app_highlevel.tex <==
% !TEX root = ../root.tex


\subsection{High-level planner}
\label{subsec:app_highlevel}

% The high-level planner preforms the optimization considering a \textit{Artistic map} ($V$) that represents the \textit{shot quality} of the possible viewpoints along the inferred actor's trajectory ($\xi_a(t)$).

% \textit{1) Viewpoint and shot definition:} Based on cinematography literature \cite{shots1}\cite{shots2}, we select a minimal set of parameters that compose most of the possible shots for single-actor, single-camera scenarios. We define a shot $\Omega_{art}$ as a set of three parameters:  $\Omega_{art}=\{\theta,\phi, r\}$, where:
% \begin{itemize}
%     \item $\theta$ is the relative yaw angle between actors direction and camera ($\theta \in [0, 2\pi]$)
%     \item $\phi$ l is the relative tilt angle between the actor’s current height plane and the camera ($\phi \in [0, \pi/2]$)
%     \item r is the shot scale which can be mapped to the distance between actor and camera ($r \in [r_{min}, r_{max}]$)
% \end{itemize}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/shot.png}
%     \caption{Shot parameters}
%     \label{fig:shot}
% \end{figure}

% \textit{2) Actor trajectory definition:} Let $\xi_a(t) : [0, t_f] \rightarrow R^3 \times SO(2)$ be the trajectory of the actor as a mapping from time to a position and heading (i.e., $\xi_a(t) = \{x_a(t), y_a(t), z_a(t), \theta_a(t)\}$), and let $\xi_a$ represent the same trajectory in a finite discrete form.

% \textit{3) Drone trajectory definition:} We assume that our drones have a gimbal controller that can orient the camera independently of the drone’s body motion. Therefore, we can purposefully decouple the drone’s heading from the main motion planning algorithm. Now, let $\xi_q(t) : [0, t_f] \rightarrow R^3$ be the trajectory of the drone as a mapping from continuous-time to a position (i.e., $\xi_q(t) = \{x_q(t), y_q(t), z_q(t)\}$), and let $\xi_q$ represent the same trajectory in a finite discrete form.

% \begin{equation}
%     \xi_q = \begin{bmatrix} p_1\\p_2\\p_3\\\vdots
%                 \end{bmatrix} = 
%                 \begin{bmatrix} p_{1x} & p_{1y} & p_{1z}\\
%                 p_{2x} & p_{2y} & p_{2z}\\
%                 p_{3x} & p_{3y} & p_{3z}\\
%                 \vdots & \vdots & \vdots
%                 \end{bmatrix}
% \end{equation}

% for a given drone $i$, let its sequence of shots be $\Omega_{qi}(t):[0:t_f] \rightarrow \Omega_{art}$ (i.e. $\Omega_{qi}(t) = {\theta_{rel}(t), \phi(t), r(t)}$). Then, the desired artistic trajectory $\xi_{shots}$ of the drone can be defined as:  

% \begin{equation}
%     \xi_{shots}(t) = T(\Omega_qi(t))
% \end{equation}
% Where $T:\Omega_{art} t[0,t_f] \rightarrow \mathbb{R}^3$, such that for a given actor's path $\xi_a$ and shot $\Omega = \{\theta, \phi, r\}$, $T(\Omega,t)$ is defined as:

% \begin{equation}
%     T(\Omega,t) = \xi_a(t) + r(t) \begin{bmatrix}
%     cos(\theta_a(t)+\theta_{rel}(t))sin(\phi(t))\\
%     sin(\theta_a(t)+\theta_{rel}(t))cos(\phi(t))\\
%     cos(\phi)
%     \end{bmatrix}
% \end{equation}

% \textit{4) state space definition:} Let $A$ be the state space of possible shots $\Omega_{art}$. Such as $A$ is a half spherical discrete domain centered and oriented on each point of the foreseen actor's path $\xi_a$, i.e. $A=\{\Omega, t \} = \{\theta_{rel}, \phi, r, t\}$ (figure  \ref{fig:state_space}). Where $n_{\theta},n_{\phi},n_{r},n_{t} \in \mathbb{N}_{>0} $ are the discretization factors of each degree of freedom.

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=0.5\linewidth]{state_space.png}
%     \caption{State space - discrete spherical domain centered on each position of the actor’s future path}
%     \label{fig:state_space}
% \end{figure}

% We tested few sets of discretization factors and achieved satisfactory results with the following values:

% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  $n_\theta = 16$ & $n_\phi = 6$ & $n_r = 6$ & $n_t = 5$  \\ 
%  \hline
% \end{tabular}
% \end{center}

% With this coordinate system, is possible to drastically reduce the complexity of the planning problem.




\section{High-level Shot quality cost function}

 % Let $V:A \rightarrow [0,1]$ be the shot quality function that maps a given shot and time to an \textit{artistic value}. $V$ applied in every region of $A$ denotes what we defined as the Artistic map. The high-level planner uses this Artistic map to optimize the camera's trajectories.  

% Considering the requirements for the system, we define $V$ a linear combination of 6 costs:
% \begin{itemize}
%     \item Shot diversity($J_d$)
%     \item Inter-drone collision ($J_{ic}$)
%     \item Inter-drone visibility one to others($J_{iv1}$)
%     \item Inter-drone visibility others to one($J_{iv2}$)
%     \item Artistic principle prior($J_{p}$)
%     \item occupancy and occlusion($J_{occ}$)
% \end{itemize}

% \begin{multline}
%     V =((1-w_d)+w_d J_d) \cdot((1-w_{ic})+w_c*W_{ic}) \cdot \\ ((1-w_{iv1})+w_{iv1} J_{iv1}) \cdot ((1-w_{iv2})+w_{iv2} J_{iv2}) \cdot \\ ((1-w_p)+w_p J_p)  \cdot ((1-w_{occ})+w_{occ} J_{occ})
% \end{multline}
% \begin{equation}
%     V = \begin{bmatrix}w_d & w_{ic} & w_{iv1} & w_{iv2} & w_{p} & w_{occ}\end{bmatrix}
%     \begin{bmatrix}
%     J_d\\
%     J_{ic}\\
%     J_{iv1}\\
%     J_{iv2}\\
%     J_{p}\\
%     J_{occ}\end{bmatrix}
% \end{equation}

% The weights of this combination are fully dependent on the application. For example, in journalistic coverage, it is probably more important to avoid inter-drone visibility than if the final application is to generate films for 3d reconstruction of the actor.

% In the following section, we are going to define each component of this cost.

% \subsection{Shot diversity cost}
% The shot diversity cost $J_d:A \rightarrow [0,1]$  was defined as a function of the absolute distance $d$ of a point $p$ in space to the position of each of the drones that have already been optimized (index $i \in [1, n_{optimized}]$).
% \begin{equation}
%     J_d(t) = \sum_{i=1}^{n_{optimized}} J_{d}'(p,\xi_{qi}(t)) 
% \end{equation}
% Where:
% \begin{equation}
%      J_{d}'(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min} \\ 
%                 d/(d_{max} - d_{min}) & \mbox{if } d_{min} < d < d_{max}\\
%                 0 & \mbox{if } d > d_{max}\end{cases}
% \end{equation} \\
% with: $d = \sqrt{(p_{1x}-p_{2x})^2+(p_{1y}-p_{2y})^2+(p_{1z}-p_{2z})^2}$\\

% This cost prevents the planner to allocate the drones too close to each other.

% \subsection{inter-drone collision cost}
% Similarly to $J_d$, the inter-drone collision cost was defined as a function of the absolute distance $d$ of a point in the space and all the drones that have already been optimized. Where
% \begin{equation}
%     J_{ic} = \sum_{i=0}^{n_{optimized}} J_{ic}(p,\xi_{qi}(t))
% \end{equation}
% Where:
% \begin{equation}
%     J_{ic}(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min}\\ 0 & \mbox{if } d > d_{min} \end{cases} 
% \end{equation}
% The distinction between $J_d$ and $J_{ic}$ is necessary to allow the control of both requirements independently.

% \subsection{Inter-drone visibility}
% The inter-drone visibility cost can be defined by 2 distinct components, (1) that checks if a given point $p$ in the space would visible by a drone that was already optimized, and (2) that checks if a drone allocated in $p$ would be able to see any of the other drones that were already optimized. 
% \begin{equation}
%     J_{iv1} = \sum_{i=0}^{n_{optimized}} J_{iv}(p,\xi_{qi}(t))
% \end{equation}
% \begin{equation}
%     J_{iv2} = \sum_{i=0}^{n_{optimized}} J_{iv}(\xi_{qi}(t),p)
% \end{equation}
% \begin{equation}
%     J_{iv}(p_1,p_2) = \begin{cases} 1 & \mbox{if } p_1 \mbox{ is visible by } p_2 \\ 0 & \mbox{otherwise}\end{cases} 
% \end{equation}

% Considering the approximation of the camera's field of view to a cone with the top angle equals to the diagonal FOV of the camera. A given point $p_1$ in the space would be visible by a shot of the actor at time $t$ from $p_2$ if 
% \begin{equation}
%     \angle (\overrightarrow{(p_2,\xi_a(t))}, \overrightarrow{(p_2,p_1)}) \leq FOV
% \end{equation}

% Assuming that the gimbal controller of the cameras keeps the actor centered in frame, then it is possible to say that the inter-drone visibility depends entirely on the position of the drones and the camera's FOV.

% Because of that, given a discrete state-space $A$, the inter-drone visibility relation between 2 points can be precomputed and stored in a matrix of $m \times m$ (where $m = n_\theta \cdot n_\phi \cdot n_r$). With that reducing the computational time demanded by each optimization cycle.


% \subsection{Occupancy and occlusion cost}
% Because of safety and artistic reasons, it is desirable that the artistic path of the drone should not be assigned inside or behind obstacles. Therefore, given an occupancy grid ($G$) of the environment, the occupancy and occlusion cost $J_{occ}$ of a shot $\Omega$ ($\Omega ={\theta_{rel}, \phi, r}$) at the time $t$ was defined as follows:

% \begin{equation}
%     J_{occ}(t) = \int_{r_{min}}^{r} G(T(\Omega,t)) d_r
% \end{equation}

% Where $G:R^3 \rightarrow [0,1]$ is a function that maps a point in space with the occupancy of the environment at that point (0 = free, 1 = occupied)

% computed in the discrete domain $A$:

% \begin{equation}
%     J_{occ}(t) = \sum_{i = 0}^{r} G'(\Omega_i,t)
% \end{equation} With:
% $i \in \mathbb{N}_{>0}$ such that $\Omega_0 = \{\Theta_{rel}, \phi, r_{min}\}$ and $\Omega_{n_r} = \{\Theta_{rel}, \phi, r_{max}\}$. 

% and

% $G': A \rightarrow [0,1]$ is the function that maps a region of the space $c$ with its relative volumetric occupancy (0 = 0\% occupied and 1=100\% occupied). The region $c$ is a section of $A$ centered in $T(\Omega,t)$ as represented by the red cell in the figure \ref{fig:state_space}.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/occ.png}
%     \caption{Occupancy and occlusion transform ($G'$) from a Cartesian occupancy grid to the artistic map domain $A$ }
%     \label{fig:occ}
% \end{figure}

% \subsection{Artistic principle cost (prior)}

% The artistic principle was defined as a user-inputted cost to penalize or give preference to specific shot types.
% For example, the figure \ref{fig:prior} represents an artistic principle that penalizes shots straight from the top. With that, the planner will avoid allocating drones in these regions.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/artistic_principle.png}
%     \caption{Example of a artistic principle (prior) that penalizes shots straight from the top, red spheres represents regions with low artistic value \abnote{(Should I change this image?)}}
%     \label{fig:prior}
% \end{figure}

% In the future works section (\ref{sec:future_work}), we discuss the possible automation of this cost, either from extracting artistic principles from existing drone filmed scenes or though image-based algorithms that learn preferred shot types, as the one described in \cite{RL_principles}.

% \section{Greedy planner}

% The high-level planner performs greedy the optimization one drone at a time based on a completely known Artistic Map (defined by the shot quality cost $V$ applied at all points of the domain $A$). 

% Initially, for the first drone, the Artistic map is computed based only on the occupancy, occlusion, and Artistic principles. Then, for the next vehicles, the artistic map is updated with the inter-drone costs. (figure \ref{fig:greedy})

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/greedy_planner.png}
%     \caption{Greedy planner over the Artistic map}
%     \label{fig:greedy}
% \end{figure}

% In order to compute the optimal path for each drone given an updated Artistic map, the planner computes the cumulative shot quality cost $V^*$ of each shot ($\Omega$) and time step, considering the next best shot ($\Omega'$) under the dynamic constraints of the drone.

% \begin{equation}
%     V^*(\Omega, t_i) = V(\omega, t_i)+min(V^*(\Omega',t_{i+1}))     
% \end{equation}
% Where, assuming the dynamic constraint that allows the drones to move only on position in the artistic domain $A$ at a time. Then for a given shot $\Omega_{ijk} = \{\theta_i, \phi_j, r_k\}$, $\Omega'$ is:
% \begin{equation}
%     \Omega'_{ijk} = \begin{bmatrix}
%         \{\theta_{i}, \phi_{j}, r_{k}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i}, \phi_{j-1}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k-1}\}\\
%     \end{bmatrix}
% \end{equation}

% \todo[inline]{Pseudo code}

==> inputs/3_app_local_planner.tex <==
% !TEX root = ../root.tex

\section{Local planner}
\label{subsec:app_local}


==> inputs/4_exp_descriptors.tex <==
% !TEX root = ../root.tex


\subsection{Learning a Descriptor Space}
\label{subsec:exp_rep}



==> inputs/4_exp_real.tex <==
% !TEX root = ../root.tex

\subsection{Real-World Results}
\label{subsec:exp_real}
\rbnote{to fill}
% \todo[inline]{experiment setup}
% \missingfigure{rviz img of the drone's path and actor's path}



jhbhjbjhbhjbjhbhjbjhbhjbjhbjhbjh
fdsfdsfs

dsfdsfdsf

2222222222222222
33333333333333333333

444444444444444

==> inputs/4_exp_sim.tex <==
% !TEX root = ../root.tex

\subsection{Simulated navigation results}
\label{subsec:exp_sim}
\rbnote{to fill}

\missingfigure{rviz img of the drone's path and actor's path, with camera view image from each drone (2 cols)}
\rbnote{to fill}

==> multidrone_icra2021 - Copy/inputs/0_abstract.tex <==
% !TEX root = ../root.tex

% \vspace{-2mm}
\begin{abstract}
Aerial cinematography is significantly expanding the capabilities of 
% professional and amateur 
film-makers.
Recent progress in autonomous unmanned aerial vehicles (UAVs) has further increased the potential impact of aerial cameras, with systems that can safely track actors in unstructured cluttered environments.
Professional productions, however, require the use of multiple cameras simultaneously to record different viewpoints of the same scene, which are edited into the final footage either in real time or in post-production.
Such extreme motion coordination is particularly hard for unscripted action scenes, which are a common use case of aerial cameras.
In this work we develop a real-time multi-UAV coordination system that is capable of recording dynamic targets while maximizing shot diversity and avoiding collisions and mutual visibility between cameras. 
We validate our approach in multiple cluttered environments of a photo-realistic simulator, and deploy the system using two UAVs in real-world experiments. 
We show that our coordination scheme has low computational cost and takes only 1.17 ms on average to plan for a team of 3 UAVs over a 10 s time horizon.
% More results can be found on the supplementary video.
Supplementary video: \url{https://youtu.be/m2R3anv2ADE}

% The task complexity only grows when we consider multi-UAV systems since, besides challenges regarding obstacle avoidance and artistic actor framing, factors as (1) shot diversity, (2) inter-drone collision, and (3) inter-drone visibility must be considered. Current approaches to control multiple aerial cameras presents severe real-life limitations, such as depending on fully scripted scenes or predefined shot types.

%  In this work we develop a system for 

% In this work, we overcome these limitations by proposing a planning system to autonomously coordinate multiple aerial cameras for partially or unscripted applications. Our approach computes sequences of desired camera views for multiple drones around a moving target, optimizing each drone’s trajectories to create diverse and artistic shots in real-time. The system was validated in a photorealistic simulator in cluttered and open environments.
% The results show that our system is able to attend all the requirements with an extremely low computational cost.

% \todo[inline]{video links}
% Supplementary video: \url{https://somelink}\\


% \rbnote{a few things to consider for abstract: - Context: What is the context of your work, what is the start of the art 
% - Need: What is the lack of the start of the art 
% - Task: What is the task you want to address in your work (should be 1 sentence) 
% - Object: How do you plan to address your task? 
% - Results: 
% - Conclusions: What are your expected conclusions?}

\end{abstract}


==> multidrone_icra2021 - Copy/inputs/1_intro.tex <==
% !TEX root = ../root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{0mm}
\section{Introduction}
\vspace{0mm}

% multi-drone filming problem
Flying cameras are revolutionizing industries that require live and dynamic camera viewpoints such as entertainment, sports, and security. 
The use of unmanned aerial vehicles (UAVs) has several advantages in comparison with traditional techniques such as dollies and cranes in terms of cost, efficiency and safety \cite{book1, santamarina2018introduction}. 
Furthermore, recent woks both in industry \cite{mavic2019,skydio2018} and academia \cite{bonatti2020autonomous,jeon2020detection,huang2018act} now allow UAVs to track targets autonomously in cluttered environments.

High-quality cinematographic productions, however, require the composition of multiple viewpoints to form the final footage \cite{bowen2013grammar,arijon1976grammar}, which can be edited \textit{on-the-fly} in the case of live sports events, or more commonly in post-production.
Camera arrangement is a complex problem that requires the production crew to reason about what is going to happen in the scene in terms of actor movements, increase viewpoint diversity, obey cinematographic guidelines (\textit{e.g.} the $180^\circ$ rule, staying on a single side of the scene), and avoid mutual visibility between cameras. 
The problem becomes even more challenging in the case of unscripted scenes in sports or journalistic coverage, where cameras need to be re-arranged more frequently while being subjected to velocity and acceleration constraints, and the event cannot be re-enacted in the case of mistakes.

Despite the large recent progress in single-UAV filming solutions, multi-UAV systems are still scarce.
Existing approaches focus mainly on coordinating vehicles to follow predefined shot types \cite{multi_drone_cine} or pre-planned filming missions \cite{events,auto_planner}, restricting the use of this technology to scripted applications.
We also find work on maximizing actor coverage \cite{coverage}, partially addressing the shot diversity objective, but this approach is restricted to 2D reasoning and static targets. 
None of the existing systems can autonomously coordinate multiple cameras in dynamic and unscripted applications.

As seen in Figure \ref{fig:main}, our work aims to tackle the full multi-UAV coordination problem, targeting cinematography in unscripted and dynamic scenarios.
We propose a system that can generate diverse and artistic shots in real-time, empowering operators with full artistic capabilities of aerial cameras. 
Our main contributions are:

\textbf{1) Problem formulation:} We formalize the multi-UAV coordination problem in term of its principal cost functions. We start with a single-UAV formulation \cite{r1} that considers trajectory smoothness, obstacle avoidance and environmental occlusions, and add new cost terms to maximize shot diversity, avoid mutual visibility between cameras, and to respect high-level user-specified cinematography guidelines;

\textbf{2) Camera coordination:} We propose a greedy framework for multi-UAV coordination that can run in real-time in dynamic scenes. First, a fast centralized planner computes a set of desired viewpoints for each camera, and a decentralized planning system computes the final trajectory for each UAV based on an occupancy map of the environment and the predicted actor trajectory;

\textbf{3) Experimental validation:} We validate our approach in multiple environments using a photo-realistic simulator, and deploy the system in real-world experiments with two UAVs.

% However, even with intelligent autonomous systems, these vehicles are susceptible to physical and dynamic constraints (speed, acceleration). Therefore, individual flying cameras often face challenges when dealing with unpredictable motions or cluttered environments. Shot diversity is also an inherent problem for single flying cameras, as long as invariant shots might appear ‘unexciting’ for the final viewer. A current solution to this problem is to record multiple takes, but it can be laborious, expensive or even infeasible in some applications. These challenges are intensified in real-world scenes, such as sports or journalistic coverage, that usually don't follow a script, and therefore cannot be reenacted. For these reasons, having access to multiple camera views can significantly improve the quality of the final video.

% current approaches overview and gap
% Currently, solutions for multi drone cinematography are scarce. Existing approaches focus mainly on coordinating vehicles to follow predefined shot types \cite{multi_drone_cine} or pre-planned filming missions \cite{events}\cite{auto_planner}, restricting the use of this technology to scripted applications. Another solution in this area focuses on maximizing the 2D coverage over static targets \cite{coverage}, partially solving the “shot diversity” problem but only in 2D and static applications. However, none of the existing systems autonomously coordinate multiple cameras in dynamic and unscripted applications.

% main contridutions
% Aiming to address this problem and empower any individual with full artistic capabilities, we propose an autonomous multi drone system to generate diverse and artistic shots in real-time. The main contributions of this work are:

% \begin{itemize}
%     \item A new framework to coordinate in real-time multiple aerial cameras. % time results
%     \item An artistic metric for multi aerial cinematographers. %validated by the user study
%     \item A high-level shot-type planner for autonomous filming drones. % real-life/ simulation tests
% \end{itemize}

% solution overview
% As input, our method combines a predefined artistic principle, for example given by a certain director style, with the occupancy map of the environment and a predicted trajectory of the actor. The optimization is done using a centralized greedy planner in an actor-centered discrete spherical domain for each time step of the foreseen actor’s path (figure \ref{fig:state_space}). For a set of optimized high-level trajectories, each drone computes its own desired trajectory by optimizing in real-time a set of cost functions using covariant gradient descent \cite{r3}. 

% validation
% Our approach was validated in a photorealistic simulator in cluttered and open environments, and tested in real life.
% An user study was performed to quantify the artistic improvement of our solution against...

==> multidrone_icra2021 - Copy/inputs/2_related_work.tex <==
% !TEX root = ../root.tex
\section{Related Work} 
\label{sec:related_work}

% \rbnote{to fill}
\textbf{Single-Drone Cinematography:}
There is vast body of academic literature and consumer products on the topic of single-drone cinematography. 
For instance, products such as the DJI Mavic \cite{mavic} and Skydio R1 \cite{skydio2018} can detect and track targets autonomously.
In addition, works such as \cite{r3, auto_1, auto_2, auto_3, auto_4, auto_5, feasible_traj} can follow user-specific artistic guidelines during motion.
We also find works that try to automate the artistic decision-making guidelines as well. For instance, \cite{RL_principles, r1} use deep reinforcement learning to train a deep policy to automatically select the best shot types for a given scene, conditioned on the current actor actions and obstacle field.
Also, \cite{huang2018act} uses the actor's skeleton configuration to automatically position the camera, maximizing the body's projection on the image.

 % targets However, depending on direct user input on unscripted applications can be challenging, demanding from the user continuous awareness of the scene to properly control the artistic guide-line that the drone should follow. This issue is intensified when scaling to a multi-drone system. The work \cite{RL_principles} successfully automates this input process using deep RL, taking a step toward a fully autonomous single-drone system.
    
    % \subsection{Multi-drone coordination}

\textbf{Multi-Robot Systems:}
There is a rich selection of work on multi-robot systems, ranging from safety and controls~\cite{luo2016distributed,luo2019multi}, planning~\cite{karnad2012modeling,jiang2019multi,liu2016mdp}, target localization~\cite{engin2020active,bayram2017tracking,charrow2014approximate}, exploration~\cite{corah2019distributed,corah2017efficient}, robot swarm task planning \cite{chandarana2018decentralized},  and even theatrical performances~\cite{cappo2018robust,cappo2018online}.
We also find important theoretical work on multi-sensor coordination using efficient greedy methods \cite{krause2008near,roberts2017submodular} that enjoy bounds on sub-optimality when compared to the full exploration of the search space.
% We find a diverse set of work on different aspects of multi-robot systems, randing from theoretical principles to more practical applications.
% For example, \cite{olfati2006flocking,zavlanos2007flocking} analyze flocking behavior on large groups of robots, \cite{luo2020behavior,chandarana2019hybrid,chandarana2018decentralized} study the behavior of robot swarms when completing multiple tasks, and other works are more focused on safety \cite{borrmann2015control,alonso2012reciprocal}.
% Other works investigate how teams of robots can collaboratively explore unknown environments \cite{corah2017efficient,corah2019communication}, perform theatrical performances \cite{cappo2018online}, and how to coordinate multiple agents using efficient greedy methods \cite{krause2008near} while still enjoying bounds on sub-optimality when compared to the full exploration of the search space. 

\textbf{Multi-Drone Cinematography:}
In the field of UAV cinematography we find a few pioneer works that employ multiple vehicles.  
For instance, \cite{multi_drone_cine} proposes an optimization-based algorithm to coordinate multiple UAVs while accounting for inter-drone collisions and mutual visibility, and requires user-defined paths as guidelines for the motion of each drone.
The work of \cite{auto_planner} takes on additional constraints into a greedy optimization, and maximizes target visibility over time using a team of drones subject to limited battery life.
\cite{coverage} simplifies the actor coverage problem to a 2D space, maximizing target visibility. 
Also focusing on multi-UAV coverage, \cite{3Dreconstruction} optimizes multiple flying cameras trajectories for efficient 3D reconstruction.
In the context of filming outdoor events with dynamic targets, \cite{events} provides an overview of cinematography principles that can be used for filming with multiple drones.

% There is a rich selection of work on multi-robot systems, ranging from safety and controls, planning, target localization, exploration, and even theatrical performances. However, multi-drones solutions applied to aerial cinematography are still scarce. 


==> multidrone_icra2021 - Copy/inputs/3_app_highlevel.tex <==
% !TEX root = ../root.tex


\subsection{High-level planner}
\label{subsec:app_highlevel}

% The high-level planner preforms the optimization considering a \textit{Artistic map} ($V$) that represents the \textit{shot quality} of the possible viewpoints along the inferred actor's trajectory ($\xi_a(t)$).

% \textit{1) Viewpoint and shot definition:} Based on cinematography literature \cite{shots1}\cite{shots2}, we select a minimal set of parameters that compose most of the possible shots for single-actor, single-camera scenarios. We define a shot $\Omega_{art}$ as a set of three parameters:  $\Omega_{art}=\{\theta,\phi, r\}$, where:
% \begin{itemize}
%     \item $\theta$ is the relative yaw angle between actors direction and camera ($\theta \in [0, 2\pi]$)
%     \item $\phi$ l is the relative tilt angle between the actor’s current height plane and the camera ($\phi \in [0, \pi/2]$)
%     \item r is the shot scale which can be mapped to the distance between actor and camera ($r \in [r_{min}, r_{max}]$)
% \end{itemize}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/shot.png}
%     \caption{Shot parameters}
%     \label{fig:shot}
% \end{figure}

% \textit{2) Actor trajectory definition:} Let $\xi_a(t) : [0, t_f] \rightarrow R^3 \times SO(2)$ be the trajectory of the actor as a mapping from time to a position and heading (i.e., $\xi_a(t) = \{x_a(t), y_a(t), z_a(t), \theta_a(t)\}$), and let $\xi_a$ represent the same trajectory in a finite discrete form.

% \textit{3) Drone trajectory definition:} We assume that our drones have a gimbal controller that can orient the camera independently of the drone’s body motion. Therefore, we can purposefully decouple the drone’s heading from the main motion planning algorithm. Now, let $\xi_q(t) : [0, t_f] \rightarrow R^3$ be the trajectory of the drone as a mapping from continuous-time to a position (i.e., $\xi_q(t) = \{x_q(t), y_q(t), z_q(t)\}$), and let $\xi_q$ represent the same trajectory in a finite discrete form.

% \begin{equation}
%     \xi_q = \begin{bmatrix} p_1\\p_2\\p_3\\\vdots
%                 \end{bmatrix} = 
%                 \begin{bmatrix} p_{1x} & p_{1y} & p_{1z}\\
%                 p_{2x} & p_{2y} & p_{2z}\\
%                 p_{3x} & p_{3y} & p_{3z}\\
%                 \vdots & \vdots & \vdots
%                 \end{bmatrix}
% \end{equation}

% for a given drone $i$, let its sequence of shots be $\Omega_{qi}(t):[0:t_f] \rightarrow \Omega_{art}$ (i.e. $\Omega_{qi}(t) = {\theta_{rel}(t), \phi(t), r(t)}$). Then, the desired artistic trajectory $\xi_{shots}$ of the drone can be defined as:  

% \begin{equation}
%     \xi_{shots}(t) = T(\Omega_qi(t))
% \end{equation}
% Where $T:\Omega_{art} t[0,t_f] \rightarrow \mathbb{R}^3$, such that for a given actor's path $\xi_a$ and shot $\Omega = \{\theta, \phi, r\}$, $T(\Omega,t)$ is defined as:

% \begin{equation}
%     T(\Omega,t) = \xi_a(t) + r(t) \begin{bmatrix}
%     cos(\theta_a(t)+\theta_{rel}(t))sin(\phi(t))\\
%     sin(\theta_a(t)+\theta_{rel}(t))cos(\phi(t))\\
%     cos(\phi)
%     \end{bmatrix}
% \end{equation}

% \textit{4) state space definition:} Let $A$ be the state space of possible shots $\Omega_{art}$. Such as $A$ is a half spherical discrete domain centered and oriented on each point of the foreseen actor's path $\xi_a$, i.e. $A=\{\Omega, t \} = \{\theta_{rel}, \phi, r, t\}$ (figure  \ref{fig:state_space}). Where $n_{\theta},n_{\phi},n_{r},n_{t} \in \mathbb{N}_{>0} $ are the discretization factors of each degree of freedom.

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=0.5\linewidth]{state_space.png}
%     \caption{State space - discrete spherical domain centered on each position of the actor’s future path}
%     \label{fig:state_space}
% \end{figure}

% We tested few sets of discretization factors and achieved satisfactory results with the following values:

% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  $n_\theta = 16$ & $n_\phi = 6$ & $n_r = 6$ & $n_t = 5$  \\ 
%  \hline
% \end{tabular}
% \end{center}

% With this coordinate system, is possible to drastically reduce the complexity of the planning problem.




\section{High-level Shot quality cost function}

 % Let $V:A \rightarrow [0,1]$ be the shot quality function that maps a given shot and time to an \textit{artistic value}. $V$ applied in every region of $A$ denotes what we defined as the Artistic map. The high-level planner uses this Artistic map to optimize the camera's trajectories.  

% Considering the requirements for the system, we define $V$ a linear combination of 6 costs:
% \begin{itemize}
%     \item Shot diversity($J_d$)
%     \item Inter-drone collision ($J_{ic}$)
%     \item Inter-drone visibility one to others($J_{iv1}$)
%     \item Inter-drone visibility others to one($J_{iv2}$)
%     \item Artistic principle prior($J_{p}$)
%     \item occupancy and occlusion($J_{occ}$)
% \end{itemize}

% \begin{multline}
%     V =((1-w_d)+w_d J_d) \cdot((1-w_{ic})+w_c*W_{ic}) \cdot \\ ((1-w_{iv1})+w_{iv1} J_{iv1}) \cdot ((1-w_{iv2})+w_{iv2} J_{iv2}) \cdot \\ ((1-w_p)+w_p J_p)  \cdot ((1-w_{occ})+w_{occ} J_{occ})
% \end{multline}
% \begin{equation}
%     V = \begin{bmatrix}w_d & w_{ic} & w_{iv1} & w_{iv2} & w_{p} & w_{occ}\end{bmatrix}
%     \begin{bmatrix}
%     J_d\\
%     J_{ic}\\
%     J_{iv1}\\
%     J_{iv2}\\
%     J_{p}\\
%     J_{occ}\end{bmatrix}
% \end{equation}

% The weights of this combination are fully dependent on the application. For example, in journalistic coverage, it is probably more important to avoid inter-drone visibility than if the final application is to generate films for 3d reconstruction of the actor.

% In the following section, we are going to define each component of this cost.

% \subsection{Shot diversity cost}
% The shot diversity cost $J_d:A \rightarrow [0,1]$  was defined as a function of the absolute distance $d$ of a point $p$ in space to the position of each of the drones that have already been optimized (index $i \in [1, n_{optimized}]$).
% \begin{equation}
%     J_d(t) = \sum_{i=1}^{n_{optimized}} J_{d}'(p,\xi_{qi}(t)) 
% \end{equation}
% Where:
% \begin{equation}
%      J_{d}'(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min} \\ 
%                 d/(d_{max} - d_{min}) & \mbox{if } d_{min} < d < d_{max}\\
%                 0 & \mbox{if } d > d_{max}\end{cases}
% \end{equation} \\
% with: $d = \sqrt{(p_{1x}-p_{2x})^2+(p_{1y}-p_{2y})^2+(p_{1z}-p_{2z})^2}$\\

% This cost prevents the planner to allocate the drones too close to each other.

% \subsection{inter-drone collision cost}
% Similarly to $J_d$, the inter-drone collision cost was defined as a function of the absolute distance $d$ of a point in the space and all the drones that have already been optimized. Where
% \begin{equation}
%     J_{ic} = \sum_{i=0}^{n_{optimized}} J_{ic}(p,\xi_{qi}(t))
% \end{equation}
% Where:
% \begin{equation}
%     J_{ic}(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min}\\ 0 & \mbox{if } d > d_{min} \end{cases} 
% \end{equation}
% The distinction between $J_d$ and $J_{ic}$ is necessary to allow the control of both requirements independently.

% \subsection{Inter-drone visibility}
% The inter-drone visibility cost can be defined by 2 distinct components, (1) that checks if a given point $p$ in the space would visible by a drone that was already optimized, and (2) that checks if a drone allocated in $p$ would be able to see any of the other drones that were already optimized. 
% \begin{equation}
%     J_{iv1} = \sum_{i=0}^{n_{optimized}} J_{iv}(p,\xi_{qi}(t))
% \end{equation}
% \begin{equation}
%     J_{iv2} = \sum_{i=0}^{n_{optimized}} J_{iv}(\xi_{qi}(t),p)
% \end{equation}
% \begin{equation}
%     J_{iv}(p_1,p_2) = \begin{cases} 1 & \mbox{if } p_1 \mbox{ is visible by } p_2 \\ 0 & \mbox{otherwise}\end{cases} 
% \end{equation}

% Considering the approximation of the camera's field of view to a cone with the top angle equals to the diagonal FOV of the camera. A given point $p_1$ in the space would be visible by a shot of the actor at time $t$ from $p_2$ if 
% \begin{equation}
%     \angle (\overrightarrow{(p_2,\xi_a(t))}, \overrightarrow{(p_2,p_1)}) \leq FOV
% \end{equation}

% Assuming that the gimbal controller of the cameras keeps the actor centered in frame, then it is possible to say that the inter-drone visibility depends entirely on the position of the drones and the camera's FOV.

% Because of that, given a discrete state-space $A$, the inter-drone visibility relation between 2 points can be precomputed and stored in a matrix of $m \times m$ (where $m = n_\theta \cdot n_\phi \cdot n_r$). With that reducing the computational time demanded by each optimization cycle.


% \subsection{Occupancy and occlusion cost}
% Because of safety and artistic reasons, it is desirable that the artistic path of the drone should not be assigned inside or behind obstacles. Therefore, given an occupancy grid ($G$) of the environment, the occupancy and occlusion cost $J_{occ}$ of a shot $\Omega$ ($\Omega ={\theta_{rel}, \phi, r}$) at the time $t$ was defined as follows:

% \begin{equation}
%     J_{occ}(t) = \int_{r_{min}}^{r} G(T(\Omega,t)) d_r
% \end{equation}

% Where $G:R^3 \rightarrow [0,1]$ is a function that maps a point in space with the occupancy of the environment at that point (0 = free, 1 = occupied)

% computed in the discrete domain $A$:

% \begin{equation}
%     J_{occ}(t) = \sum_{i = 0}^{r} G'(\Omega_i,t)
% \end{equation} With:
% $i \in \mathbb{N}_{>0}$ such that $\Omega_0 = \{\Theta_{rel}, \phi, r_{min}\}$ and $\Omega_{n_r} = \{\Theta_{rel}, \phi, r_{max}\}$. 

% and

% $G': A \rightarrow [0,1]$ is the function that maps a region of the space $c$ with its relative volumetric occupancy (0 = 0\% occupied and 1=100\% occupied). The region $c$ is a section of $A$ centered in $T(\Omega,t)$ as represented by the red cell in the figure \ref{fig:state_space}.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/occ.png}
%     \caption{Occupancy and occlusion transform ($G'$) from a Cartesian occupancy grid to the artistic map domain $A$ }
%     \label{fig:occ}
% \end{figure}

% \subsection{Artistic principle cost (prior)}

% The artistic principle was defined as a user-inputted cost to penalize or give preference to specific shot types.
% For example, the figure \ref{fig:prior} represents an artistic principle that penalizes shots straight from the top. With that, the planner will avoid allocating drones in these regions.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/artistic_principle.png}
%     \caption{Example of a artistic principle (prior) that penalizes shots straight from the top, red spheres represents regions with low artistic value \abnote{(Should I change this image?)}}
%     \label{fig:prior}
% \end{figure}

% In the future works section (\ref{sec:future_work}), we discuss the possible automation of this cost, either from extracting artistic principles from existing drone filmed scenes or though image-based algorithms that learn preferred shot types, as the one described in \cite{RL_principles}.

% \section{Greedy planner}

% The high-level planner performs greedy the optimization one drone at a time based on a completely known Artistic Map (defined by the shot quality cost $V$ applied at all points of the domain $A$). 

% Initially, for the first drone, the Artistic map is computed based only on the occupancy, occlusion, and Artistic principles. Then, for the next vehicles, the artistic map is updated with the inter-drone costs. (figure \ref{fig:greedy})

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/greedy_planner.png}
%     \caption{Greedy planner over the Artistic map}
%     \label{fig:greedy}
% \end{figure}

% In order to compute the optimal path for each drone given an updated Artistic map, the planner computes the cumulative shot quality cost $V^*$ of each shot ($\Omega$) and time step, considering the next best shot ($\Omega'$) under the dynamic constraints of the drone.

% \begin{equation}
%     V^*(\Omega, t_i) = V(\omega, t_i)+min(V^*(\Omega',t_{i+1}))     
% \end{equation}
% Where, assuming the dynamic constraint that allows the drones to move only on position in the artistic domain $A$ at a time. Then for a given shot $\Omega_{ijk} = \{\theta_i, \phi_j, r_k\}$, $\Omega'$ is:
% \begin{equation}
%     \Omega'_{ijk} = \begin{bmatrix}
%         \{\theta_{i}, \phi_{j}, r_{k}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i}, \phi_{j-1}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k-1}\}\\
%     \end{bmatrix}
% \end{equation}

% \todo[inline]{Pseudo code}

==> multidrone_icra2021 - Copy/inputs/3_app_local_planner.tex <==
% !TEX root = ../root.tex

\section{Local planner}
\label{subsec:app_local}


==> multidrone_icra2021 - Copy/inputs/3_approach.tex <==
% !TEX root = ../root.tex

\section{Multi-Camera Coordination} 
\label{sec:approach}

We now detail the methods we use for camera coordination in the multi-UAV system.
As displayed in Equation~\ref{eq:main_cost}, our overall objective function involves the minimization of $6$ sub-objectives, which often conflict with one another. 
Our goal is to formulate an algorithm that works in real-time, in unscripted scenes, and that can deal with a state space which grows exponentially in complexity with the number of UAVs. 
Given this challenge, we prefer to find fast solutions which are only locally optimal as opposed to globally optimal trajectories that take a long time to compute.

To address the time complexity issue, we break down our method into three main subsystems that operate together.
First, a centralized motion planner (Sec.~\ref{subsec:centralized}) coordinates desired positions for all cameras simultaneously.
Next, a decentralized motion planner network (Sec.~\ref{subsec:decentralized}) computes the final trajectories for each specific UAV.
Finally, an image selection module (Sec.~\ref{subsec:img_selection}) chooses the best live image to be displayed out of all cameras. 
Alternatively, the final image selection can be manually performed in post-production. 
Fig.~\ref{fig:system} depicts the system diagram.

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/diagram.png}
    \caption{\small System overview: a centralized waypoint planner computes discrete camera positions. Next, a decentralized planning system optimizes smooth trajectories for each UAV.
    \vspace{-3mm}}
    \label{fig:system}
\end{figure}

\subsection{Centralized Multi-Camera Planning}
\label{subsec:centralized}

Our centralized planning system parametrizes trajectories as waypoints, i.e., $\Path{} \in \real^{T \times 3}$, where $T$ is the number of time steps. 
We assume that the heading dimension $\psi(t)$ is set to always point the drone from $\Path{qi}(t)$ towards the actor in $\Path{a}(t)$, which can be achieved independently of the aircraft's translation by rotating the UAV's body and camera gimbal.
We parametrize the state-space of all possible camera positions using spherical coordinates $\{\rho, \theta, \phi\}$ centered on the actor's location: 
\vspace{-4mm}

\begin{equation}
	\begin{aligned}
		&\Path{qi}(t) = \Path{a}(t) + \rho 
		\begin{bmatrix}
		 cos(\psi_a + \theta) sin(\phi)\\
		 sin(\psi_a + \theta) cos(\phi)\\
		 cos(\phi)
		\end{bmatrix}\\
	\end{aligned}
\end{equation}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\linewidth]{state_space.png}
%     \caption{State space - discrete spherical domain centered on each position of the actor’s future path \rbnote{remove path or make it more clear. better use of space in figure? too much empty space. maybe put the whole lattice (artistic prior) with it as A and B } \abnote{maybe it could be displayed side by side with the equation above}}
%     \label{fig:state_space}
% \end{figure}


\textbf{Space discretization: } 
We define a discrete state-space lattice $S$ that contains all possible camera positions distributed as $|S| = 576$ points in a half-sphere above ground.
\begin{wrapfigure}{r}{0.45\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/state_space}
    \caption{\small Discrete spherical state space centered on actor.
    \vspace{-2mm}}
    \label{fig:state_space}
\end{wrapfigure}
Based on cinematographic guidelines \cite{arijon1976grammar,bowen2013grammar} we equally divide the yaw coordinates $\theta$ into $16$ values between $[0, 2\pi]$, the tilt angles $\phi$ into $6$ values between $[0, \pi/2]$, and the distance to actor within the set $\rho \subseteq \{2, 3, 4, 5, 6, 7\}$, ranging from close-up to long shots. 
In addition, we discretize the trajectory's time into $5$ steps equally spaced every $2$ seconds, forming a $10$-second planning time horizon.


\textbf{Cost functions: }
Next we mathematically formulate the cost functions that optimized by the centralized camera planner for the set of UAV trajectories $\Xi$: 

% Let $V:A \rightarrow [0,1]$ be the shot quality function that maps a given shot and time to an \textit{artistic value}. $V$ applied in every region of $A$ denotes what we defined as the Artistic map. The high-level planner uses this Artistic map to optimize the camera's trajectories.  

\textit{i) Shot diversity cost: }
The shot diversity cost prevents the planner to allocate the $n$ camera positions close to each other up until a maximum distance $d_{max}^{div}$:
\vspace{-0mm}
\begin{equation}
\label{eq:cost_div}
\begin{aligned}
    &\costFnDiv{\Xi} = \sum_{\tau=1}^{T} \sum_{i=1}^{n} \sum_{j=1}^{n} D({\Path{qi}(\tau), \Path{qj}(\tau)}),\\
    \text{where} \quad & D(p_1,p_2) = 
    	\begin{cases} 
    		1 & \mbox{if } d < d_{min}^{div} \\ 
            \frac{d}{d_{max}^{div} - d_{min}^{div}} & \mbox{if } d_{min}^{div} < d < d_{max}^{div}\\
            0 & \mbox{if } d > d_{max}^{div}
        \end{cases}
\end{aligned}
\end{equation}

% $\costFnDiv{\Xi} = \sum_{i=1}^{n} \Path{qi} \rightarrow [0,1]$ was defined as a function of the absolute distance $d$ of a point $p$ in space to the position of each of the drones that have already been optimized (index $i \in [1, n_{optimized}]$).

% \begin{equation}
%     J_d(t) = \sum_{i=1}^{n_{optimized}} J_{d}'(p,\xi_{qi}(t)) 
% \end{equation}
% Where:
% \begin{equation}
%      J_{d}'(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min} \\ 
%                 d/(d_{max} - d_{min}) & \mbox{if } d_{min} < d < d_{max}\\
%                 0 & \mbox{if } d > d_{max}\end{cases}
% \end{equation} \\
% with: $d = \sqrt{(p_{1x}-p_{2x})^2+(p_{1y}-p_{2y})^2+(p_{1z}-p_{2z})^2}$\\

% This cost prevents the planner to allocate the drones too close to each other. 

\textit{ii) Inter-drone collision cost: }
Analogously to $\costDiv$ in Eq.~\ref{eq:cost_div}, we define the inter-drone collision cost as a measure of distance between UAVs. 
The user can, however, choose a different cost weight $\lambda$ and safety distance $d_{max}^{col}$ to penalize collisions. 


% was defined as a function of the absolute distance $d$ of a point in the space and all the drones that have already been optimized. Where
% \begin{equation}
%     J_{ic} = \sum_{i=0}^{n_{optimized}} J_{ic}(p,\xi_{qi}(t))
% \end{equation}
% Where:
% \begin{equation}
%     J_{ic}(p_1,p_2) = \begin{cases} 1 & \mbox{if } d < d_{min}\\ 0 & \mbox{if } d > d_{min} \end{cases} 
% \end{equation}
% The distinction between $J_d$ and $J_{ic}$ is necessary to allow the control of both requirements independently.

\textit{iii) Inter-drone visibility:}
We express the inter-drone visibility cost as a binary measure $V(p_i,p_j) \subseteq \{0,1\}$ of whether point $j$ is visible from position $i$.
We model the visible area as a cone in space using the camera's diagonal field-of-view angle, and position its center line towards the actor's position:
\vspace{-2mm}
\begin{equation}
\label{eq:cost_vis}
    \costFnVis{\Xi} = \sum_{\tau=1}^{T} \sum_{i=1}^{n} \sum_{j=1}^{n} V({\Path{qi}(\tau), \Path{qj}(\tau)})
    \vspace{-2mm}
\end{equation}

We pre-compute all mutual visibility values into a look-up table to reduce planning times, which is possible in our discrete state-space model.

% The inter-drone visibility cost can be defined by 2 distinct components, (1) that checks if a given point $p$ in the space would visible by a drone that was already optimized, and (2) that checks if a drone allocated in $p$ would be able to see any of the other drones that were already optimized. 
% \begin{equation}
%     J_{iv1} = \sum_{i=0}^{n_{optimized}} J_{iv}(p,\xi_{qi}(t))
% \end{equation}
% \begin{equation}
%     J_{iv2} = \sum_{i=0}^{n_{optimized}} J_{iv}(\xi_{qi}(t),p)
% \end{equation}
% \begin{equation}
%     J_{iv}(p_1,p_2) = \begin{cases} 1 & \mbox{if } p_1 \mbox{ is visible by } p_2 \\ 0 & \mbox{otherwise}\end{cases} 
% \end{equation}

% Considering the approximation of the camera's field of view to a cone with the top angle equals to the diagonal FOV of the camera. A given point $p_1$ in the space would be visible by a shot of the actor at time $t$ from $p_2$ if 
% \begin{equation}
%     \angle (\overrightarrow{(p_2,\xi_a(t))}, \overrightarrow{(p_2,p_1)}) \leq FOV
% \end{equation}

% Assuming that the gimbal controller of the cameras keeps the actor centered in frame, then it is possible to say that the inter-drone visibility depends entirely on the position of the drones and the camera's FOV.

% Because of that, given a discrete state-space $A$, the inter-drone visibility relation between 2 points can be precomputed and stored in a matrix of $m \times m$ (where $m = n_\theta \cdot n_\phi \cdot n_r$). With that reducing the computational time demanded by each optimization cycle.


\textit{iv) Obstacle and occlusion avoidance: }
In order to keep all UAVs safe and to maintain visibility of the actor at all times, we must reason about the role of obstacles in the environment.
First, we transform the environment's occupancy grid into a time-dependent spherical domain centered around the actor $\grid \rightarrow \grid_{s}^{t} \in [0,1]$, as shown in Fig.~\ref{fig:grid_sphere}. We then compute the obstacle avoidance cost by summing the occupancy likelihood of all cells within a radius $r_{max}$ of each UAV. We also calculate the occlusion cost as a measure of occupancy along a line $l_i(\tau) = \tau\Path{qi}(t) + (1-\tau)\Path{a}(t)$ between UAV and actor:
\vspace{-5mm}

\begin{equation}
\begin{aligned}
\label{eq:cost_obs_and_occ}
    \costFnObs{\Xi} &= \sum_{\tau=1}^{T} \sum_{i=1}^{n} \int_0^{r_{max}} \grid_{s}^{\tau}({\Path{qi}(\tau)}) \ d(\text{volume})\\
    \costFnOcc{\Xi} &= \sum_{\tau=1}^{T} \sum_{i=1}^{n} \int_0^{1}\grid_{s}^{\tau}({l_i(\tau)}) \ d\tau
    \vspace{-2mm}
\end{aligned}
\end{equation}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/raw/occupancy_obstacle_artistic_map.png}
%     \caption{Occupancy and occlusion transform ($G'$) from a Cartesian occupancy grid to the artistic map domain $A$ 
%     \rbnote{change caption. improve figure. use helvetica as font. why is there gray on circular grid if there's only black in euclidian space?}}
%     \label{fig:grid_sphere}
% \end{figure}





% Because of safety and artistic reasons, it is desirable that the artistic path of the drone should not be assigned inside or behind obstacles. Therefore, given an occupancy grid ($G$) of the environment, the occupancy and occlusion cost $J_{occ}$ of a shot $\Omega$ ($\Omega ={\theta_{rel}, \phi, r}$) at the time $t$ was defined as follows:

% \begin{equation}
%     J_{occ}(t) = \int_{r_{min}}^{r} G(T(\Omega,t)) d_r
% \end{equation}

% Where $G:R^3 \rightarrow [0,1]$ is a function that maps a point in space with the occupancy of the environment at that point (0 = free, 1 = occupied)

% computed in the discrete domain $A$:

% \begin{equation}
%     J_{occ}(t) = \sum_{i = 0}^{r} G'(\Omega_i,t)
% \end{equation} With:
% $i \in \mathbb{N}_{>0}$ such that $\Omega_0 = \{\Theta_{rel}, \phi, r_{min}\}$ and $\Omega_{n_r} = \{\Theta_{rel}, \phi, r_{max}\}$. 

% and

% $G': A \rightarrow [0,1]$ is the function that maps a region of the space $c$ with its relative volumetric occupancy (0 = 0\% occupied and 1=100\% occupied). The region $c$ is a section of $A$ centered in $T(\Omega,t)$ as represented by the red cell in the figure \ref{fig:state_space}.

\textit{v) Cinematography guidelines as cost prior: }
We also allow operators to manually specify a cost prior $\costCine$ for each cell, in case they wish to follow specific cinematographic guidelines. 
For example, Fig.~\ref{fig:prior_overhead} shows an example where we define overhead shots as undesired.

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.47\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/raw/occupancy_obstacle_artistic_map.png}
         \caption{}
         \label{fig:grid_sphere}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.51\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/prior_y12_p5_r3_rmin2_rmax5.png}
         \caption{}
         \label{fig:prior_overhead}
     \end{subfigure}
        \caption{\small
        (a) Visualization of occupancy and occlusion avoidance costs in the cells of the spherical grid $\grid_{s}^{t}$.
        (b) Example of a cinematography guideline prior that penalizes overhead shots. Red  spheres  represent  regions of high cost.
        \vspace{-5mm}}
        \label{fig:three graphs}
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figs/prior_y12_p5_r3_rmin2_rmax5.png}
%     \caption{Example of a artistic principle (prior) that penalizes shots straight from the top, red spheres represents regions with low artistic value \rbnote{remove orange line from figure}
%     \vspace{-4mm}}
%     \label{fig:prior}
% \end{figure}


% The artistic principle was defined as a user-inputted cost to penalize or give preference to specific shot types.
% For example, the figure \ref{fig:prior} represents an artistic principle that penalizes shots straight from the top. With that, the planner will avoid allocating drones in these regions.

\textbf{Greedy optimization: }
The centralized planning problem for multi-camera optimization over multiple time steps proves to be NP-hard, similarly to other optimal sensor placement works \cite{greedy1,krause2006near,arora2017randomized}.
In order to make the computation tractable in real-time and avoid a combinatorial problem, we develop a greedy optimization approach that computes the optimal trajectory 
$\Path{q\,i}^{*\text{greedy}}$
for each UAV sequentially, fixing all previously calculated trajectories 
$\{ \Path{q\,1}^{*\text{greedy}}$, ..., $\Path{q\,i-1}^{*\text{greedy}} \}$. 
% \rbnote{if we have time, try to prove that this falls under the monotonic submodular category, so we have sub-optimality guarantees -- how bad we can be compared to optimal planner}

\begin{wrapfigure}{r}{0.45\linewidth}
% \begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{figs/greedy.png}
    \caption{\small Greedy planner.
    \vspace{-4mm}}
    \label{fig:greedy}
% \end{figure}
\end{wrapfigure}

At each stage $i$ we employ a backward induction dynamic programming algorithm \cite{sutton2018reinforcement,bertsekas1995dynamic,lavalle2006planning} to find the optimal cost-to-go for of each state $s \subseteq S$ at all time steps, analogously to a value iteration algorithm.
To do so, we build a cost map $C: S \rightarrow \real^{|S|}$ that contains the cost of all states, and a cost-to-go map $V: S \rightarrow \real^{|S|}$.
In order to make transitions between cells dynamically feasible for the real vehicle, we only allow expansions to neighboring cells in the spherical grid.
Since we operate in a discrete state-space with a small branching factor and deterministic transitions, a single backwards pass quickly yields the optimal solution.
Finally, we build the full trajectory $\Path{q\,i}^{*\text{greedy}}$ by selecting neighboring cells with the least cost-to-go at consecutive time steps, starting at the UAV's initial position $S_i^0$.
We update the cost manifold after each drone is added, since inter-visibility, shot diversity, and collision costs are recalculated. 
Algorithm~\ref{alg:greedy_alg} details the process:

\small
\begin{algorithm}[ht]
\caption{\small Compute greedy traj. set $\Xi = \{\Path{q1}, ..., \Path{qn} \}$}
\label{alg:greedy_alg}
\SetAlgoLined
 Initialize $\Xi_{\textnormal{greedy}} = \{\}$ \Comment{\footnotesize empty set}
 \For{\textnormal{\textbf{each}} \textnormal{UAV} $i$}{
  $C$ $\gets$ $J(S, \Xi_{\textnormal{greedy}})$ \Comment{\footnotesize update entire cost map}
  $V$ $\gets$ Backward\_Induction($C$) \Comment{\scriptsize update cost-to-go}
  $\Path{q\,i}^{*\text{greedy}}$ $\gets$ Optimal\_Path($V$, $S_i^0$)\;
  Append $\Path{q\,i}^{*\text{greedy}}$ to $\Xi_{\textnormal{greedy}}$\;
 }
 \textbf{return} $\Xi_{\textnormal{greedy}}$
\end{algorithm}
\vspace{-3mm}
\normalsize




% The high-level planner performs greedy the optimization one drone at a time based on a completely known Artistic Map (defined by the shot quality cost $V$ applied at all points of the domain $A$). 

% Initially, for the first drone, the Artistic map is computed based only on the occupancy, occlusion, and Artistic principles. Then, for the next vehicles, the artistic map is updated with the inter-drone costs. (figure \ref{fig:greedy})



% In order to compute the optimal path for each drone given an updated Artistic map, the planner computes the cumulative shot quality cost $V^*$ of each shot ($\Omega$) and time step, considering the next best shot ($\Omega'$) under the dynamic constraints of the drone.

% \begin{equation}
%     V^*(\Omega, t_i) = V(\omega, t_i)+min(V^*(\Omega',t_{i+1}))     
% \end{equation}
% Where, assuming the dynamic constraint that allows the drones to move only on position in the artistic domain $A$ at a time. Then for a given shot $\Omega_{ijk} = \{\theta_i, \phi_j, r_k\}$, $\Omega'$ is:
% \begin{equation}
%     \Omega'_{ijk} = \begin{bmatrix}
%         \{\theta_{i}, \phi_{j}, r_{k}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j}, r_{k+1}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k}\}\\
%         \{\theta_{i+1}, \phi_{j+1}, r_{k+1}\}\\
%         \{\theta_{i}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i}, \phi_{j-1}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j}, r_{k-1}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k}\}\\
%         \{\theta_{i-1}, \phi_{j-1}, r_{k-1}\}\\
%     \end{bmatrix}
% \end{equation}


\subsection{Decentralized UAV Trajectory Optimization and Tracking}
\label{subsec:decentralized}

After calculating the greedy-optimal set of UAV trajectories $\Xi_{\textnormal{greedy}}$ using the centralized planner, we post-process each output using a decentralized planning system.
Our objective here is to obtain smoother individual trajectories at a finer time discretization. 
While the original waypoints were spaced every $2$ seconds over a $10$-second horizon, here we achieve finer resolutions with $0.5$ s granularity in local planning, and $0.02$ s for trajectory tracking.
We employ the single-UAV local planner described in \cite{r1}, which uses covariant gradient descent to produce locally optimal trajectories while considering the costs of smoothness, obstacle and occlusions avoidance, and a desired artistic trajectory, which we define as $\Path{q\,i}^{*\text{greedy}}$. 
In addition, each local planner receives the expected waypoints of all remaining vehicles, and avoids positioning its trajectory within 1m of other UAVs.
We run the local planner at $5$ Hz, and use a PID controller at $50$ Hz.
\vspace{-0mm}

\subsection{Live Image Selection}
\label{subsec:img_selection}
\vspace{-0mm}
Even though our system produces multiple image streams, most filming applications display a single camera to the viewer at a time.
The final movie can be produced with manual post-processing, or in the case of live streams it requires a human to make selections while viewing all videos simultaneously.
Here, we propose a method for automatic selection of live images based on a subset of our cost functions. 
We compute a image quality score $Q_i$ for each camera stream, calculated as a weighted sum of the inter-drone visibility cost $\costVis$ and of the prior cinematographic guidelines $\costCine$. 
We select the current camera with the highest score, and once a camera is chosen we exponentially decay its score to foster viewpoint diversity, and gradually return it to the original value once another image is chosen.
Based on cinematography literature we set minimum and maximum limits for shot lengths of $3$ and $8$ seconds respectively, which are reasonable units of length for individual action shots \cite{mahadani_mahadanii_2015,cutting2010attention}.

% The multi-camera problem can be divided into 2 main steps: (1) Generating the videos and (2) editing them. The first one consists of a np-hard optimization problem, and because of that, an optimal path for the cameras can not be guaranteed in a reasonable time. But, assuming that quality of all possible viewpoints of the actor can be described as a \textit{shot quality} function, and that this function is monotonic and submodular, a greedy placement of the cameras has bounded sub-optimality guarantees\cite{greedy1}\cite{greedy2}. The second part of the problem consists of choosing a shot sequence among the generated videos. To do that a few artistic principles must be taken into considerations: first, the selected videos must have a good \textit{shot quality}, and second, the transition between viewpoints must be pleasurable (e.g avoid too fast transition and also monotonous continuous viewpoints).

% The \textit{shot quality} function is qualitative and directly related to the Artistic principle followed and the spectator's taste. However, the cinematography literature presents several guidelines that can help to quantify the quality of a shot \cite{shots1}\cite{shots2} and the transitions between them.

% Considering these artistic guidelines and safety concerns, we established a few requirements for the multi drone system:

% \begin{enumerate}
% \item Must explore shot diversity
% \item Must avoid Inter-drone visibility
% \item Must avoid obstacles collision and occlusion 
% \item Must avoid Inter-drone collision 
% \item Must consider artistic inputs from the user
% \end{enumerate}

% In this work, we propose a multi drone system capable of coordinating multiple aerial cameras around a moving actor in cluttered environments without any scripts.

% \input{inputs/3_app_highlevel}
% \input{inputs/3_app_local_planner}


% \todo[inline]{local optimization and (interdrone) costs formulation }




==> multidrone_icra2021 - Copy/inputs/3_problem_formulation.tex <==
% !TEX root = ../root.tex

\section{Problem formulation} 
\label{sec:problem_formulation}

Our overall task is to optimally control a team of UAVs to film an actor who is moving through an environment with obstacles. 
Similarly to \cite{r1}, we formulate a trajectory optimization problem using cost functions that measure environmental occlusion of the actor, jerkiness of motion and safety. In addition, we introduce new cost components for maximizing shot diversity between UAVs, avoid inter-vehicle visibility, and to allow user-specified cinematographic guidelines.

Let $\Path{qi} : [0,t_f] \rightarrow \real^3  \times SO(2)$ be the trajectory of the \textit{i}-th UAV, i.e., $\Path{qi}(t) = \{x(t), y(t), z(t), \psi_{q}(t)\}$, and $\Xi = \{\Path{q1}, ..., \Path{qn} \}$ be the set of trajectories from $n$ UAVs.
Let $\Path{a} : [0,t_f] \rightarrow \real^3  \times SO(2)$ be the trajectory of the actor, $\Path{a}(t) = \{x(t), y(t), z(t), \psi_{a}(t)\}$, which is inferred using the onboard cameras.
Let grid $\grid: \real^3 \rightarrow [0, 1]$ be a voxel occupancy grid that maps every point in space to a probability of occupancy. Let $\map : \real^3 \rightarrow \real$ be the signed distance values of a point to the nearest obstacle. 
% Positive sign is for points in free space, and negative sign is for points either in occupied or unknown space, which we assume to be potentially inside an obstacle.
Our mathematical objective is to minimize a cost function $\costFn{\Xi}$ that tends to the following objectives:

\textit{1) Smoothness:} Penalizes jerky motions that may lead to camera blur and unstable flight. Calculated as the sum of costs from individual trajectories:
$\costFnSmooth{\Xi} = \sum_i \costFnSmooth{\Path{qi}}$\\
\textit{2) Occlusion:} Penalizes occlusion of the actor by obstacles in the environment for each camera:
$\costFnOcc{\Xi} = \sum_i \costFnOcc{\Path{qi},\Path{a},\map}$\\
\textit{3) Safety:} Penalizes proximity to obstacles that are unsafe for each UAV:
$\costFnObs{\Xi} = \sum_i \costFnObs{\Path{qi},\map}$\\
\textit{4) Diversity:} Penalizes viewpoints similarities between UAVs. Calculated over the entire set of trajectories:
$\costFnDiv{\Xi,\Path{a}}$\\
\textit{5) Inter-visibility:} Avoids visibility between UAVs:
$\costFnVis{\Xi}$\\
\textit{6) Cinematography guidelines:} Penalizes user-specified undesired viewpoints (\textit{e.g.} high tilt angles):
$\costFnCine{\Xi,\Path{a}}$

We then compose the overall cost function as a linear combination between each component, with relative weights $\lambda$.
The solution $\Xi^*$ is then tracked by each UAV:
\vspace{-2mm}

\begin{equation}
\begin{aligned}
\label{eq:main_cost}
\costFn{\Xi} &=  \begin{bmatrix}
       1 & \lambda_1 & \lambda_2 & \lambda_3 & \lambda_4 & \lambda_5
     \end{bmatrix} 
\begin{bmatrix}
       \costFnSmooth{\Xi} \\
       \costFnOcc{\Xi} \\
       \costFnObs{\Xi} \\
       \costFnDiv{\Xi}\\
       \costFnVis{\Xi}\\
       \costFnCine{\Xi}
     \end{bmatrix} \\
%\costFnSmooth{\Path{q}} + \lambda_1 \costFnObs{\Path{q}} + \lambda_2 \costFnOcc{\Path{q},\Path{a}} + \lambda_3 \costFnShot{\Path{q},\Path{a}} \\
\Xi^* &= \argminprob{} \quad \costFn{\Xi}
\end{aligned}
\end{equation}
\vspace{-2mm}





% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/overall.png}
%     \caption{Overall architecture }
%     \label{fig:overall}
% \end{figure*}



==> multidrone_icra2021 - Copy/inputs/4_exp.tex <==
% !TEX root = ../root.tex
\section{Experimental Results} 
\label{sec:results}
Here we detail the simulated and real-world experiments that validate our multi-UAV cinematography system. 
Additional visualizations are shown in the supplementary video.

\subsection{Simulation experiments}
\label{subsec:exp_sim}

\textbf{Experimental setup: }
We record all simulated data using a drone in a photo-realistic environment,
AirSim \cite{shah2018airsim}, coupled with a custom ROS interface \cite{ros}. 
As seen in the supplementary video, our simulated scenes consists of
an animated character walking around a suburban environment, surrounded by obstacles such as trees, buildings, and posts.

\begin{figure*}[]
     \centering
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/sim_rural.png}
         \caption{}
         \label{fig:env_rural}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/sim_neighborhood.png}
         \caption{}
         \label{fig:env_city}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/sim_forest.png}
         \caption{}
         \label{fig:env_forest}
     \end{subfigure}
        \caption{\small Diverse range of simulated environments where we tested our multi-UAV system: a) narrow gaps, b) suburban environment with sparse tall obstacles, and c) dense foliage.
        \vspace{-4mm}}
        \label{fig:three_envs}
\end{figure*}

\textbf{E1) Viewpoint diversity validation: }
This first experiment's objective was to validate the assumption of the relation between shot diversity and artistic quality by quantifying the benefits of the employing multiple UAVs for aerial cinematography as opposed to the use of a single camera.
To do so, we generated a set of $5$ videos with $12$ seconds of length of an actor walking around a park.
The first clip featured a single-camera back shot for its entire duration, while all other clips alternated between the back shot and a secondary viewpoint every $3$ seconds. 
We chose the secondary viewpoints to be either $45^{\circ}$, $90^{\circ}$, $135^{\circ}$, or $180^{\circ}$ for each of the other four videos respectively. 

For this survey we recruited $15$ participants using Amazon Mechanical Turk (MTurk) \cite{turkamazon}, who were compensated for their time.
After being approved on a short qualifying task, each participant viewed a total of 12 pairs of videos, one being the constant back shot clip, and the other being one of the multi-viewpoint clips. 
Videos were played synchronously three times, and after watching at least once participants answered: ``\textit{Which video is more enjoyable?}''
Each clip was compared 15 times against the baseline single-camera shot.

Figure \ref{fig:shot_diversity} displays the survey results, where the height of each bar represents the percentage of users that rated the multi-UAV clip as being more enjoyable than the single-UAV clip.
As expected, we found that an overwhelming majority of users prefer to watch a scene with viewpoint diversity.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/shot_diversity_.png}
    \caption{\small User study to evaluate viewer preference for videos with diverse viewpoints. We ask users to compare how enjoyable a single back shot view is against clips with additional viewpoints. Vertical bar shows percentage of users that prefer the video with a secondary viewpoint, where each bar corresponds to an angle value.
    \vspace{-2mm}}
    \label{fig:shot_diversity}
\end{figure}

\textbf{E2) Robustness across environments: }
We tested our approach in a diverse set of photo-realistic simulations, ranging from open to cluttered environments, and with groups of UAVs containing 2 to 5 vehicles. 
As shown in Figure \ref{fig:three_envs}, our approach is able to successfully coordinate the teams of UAVs in a wide spectrum of scenarios.  
For instance, in \ref{fig:env_rural} the actor passes trough a narrow gap (2m) that the UAVs need to avoid, and in \ref{fig:env_city} she walks next to a extensive line of trees (1m apart), which forces the UAVs to move to the right side of the actor. In addition, in \ref{fig:env_forest} we see the UAVs navigating within dense and unstructured foliage tunnels.
 
The tests indicate that our system is able to adapt to a diverse range of environments and actor motions. Furthermore, we verify that the final clips follow our objective functions and present diverse viewpoints with little inter-drone visibility.

\textbf{E3) Scaling performance: }
We conducted a set of experiments to quantify our centralized planner's performance as it scales to larger teams of UAVs and larger state-spaces. 
This analysis is important because keeping low computational costs is vital for real-time performance.

First, we measured the planning time and computer resources consumption for finer discretizations of the state space (Table \ref{table:performance}).
We note that memory usage grows proportionally to the square of the number of cells in the state space because we employ a precomputed lookup table for the inter-drone visibility and shot diversity costs. 
However, our implementation offers large benefits in terms of computing time and CPU usage, which grow linearly.

\begin{table}[ht]
\centering
\begin{tabular}{ll|lll}
\begin{tabular}[c]{@{}l@{}}State space\\ ($n_{\psi}$,$n_{\phi}$,$n_{\rho}$)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Computed\\ states\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Planning time\\ for 3 drones [ms]\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CPU[\%]\\ (1 core)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Memory\\ use [MB] \end{tabular} \\ \cline{1-5}
(3,3,8)    & {\color[HTML]{000000} 360} & 0.17+-0.03   & 22  & 35    \\
(16,6,6)   & 2880                       & 1.17+-0.18   & 25  & 37.5  \\
(24,9,9)   & 9720                       & 4.65+-0.47   & 28  & 64    \\
(32,12,12) & 23040                      & 16.70+-1.26  & 34  & 197   \\
(40,15,15) & 45000                      & 19.56+-0.83  & 38  & 655   \\
(48,18,18) & 77760                      & 51.71+-2.04  & 52  & 1840  \\
(52,21,21) & 114660                     & 116.28+-6.98 & 75  & 4693  \\
(64,24,24) & 184320                     & 228.01+-8.85 & 100 & 10150
\end{tabular}
\caption{\small Performance of the greedy planner for different discretizations of the State space. We use 3 UAVs with a 5 time-steps horizon, and re-plan at 5 Hz. \label{table:performance}}
\end{table}

The discretization we use for most of our experiments ($n_{\psi}$=16,$n_{\phi}$=6 and $n_{\rho}$=6) presents a great trade-off, with a reasonable space discretization and a low computation time of 1.17ms, while only consuming 37.5 MB of RAM.
As a comparison, we implemented an optimal brute-force planner and tested it using the same spatial discretization and number of drones. 
Using only 2 time steps, the non-greedy planner took 16.4 seconds to find the optimal solution. The planning time jumps to 2h:30min when we consider 3 time steps. These results show the importance of adopting a greedy strategy to solve a NP-hard problem in real-time.

We also evaluated how the planning time increase with a larger number of drones and time steps. 
As expected, our greedy solution has a linear growth of complexity (Fig.~\ref{fig:time_charts}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/chart_computing_time.png}
    \caption{\small Time required by the high-level planner to compute the trajectories of the drones: (a) given the number of vehicles, (b) given the number of time steps computed an (c) given the number of states in the artistic domain ($n_{\psi} \cdot n_{\phi} \cdot n_{\rho} \cdot n_t$)
    \vspace{-3mm}}
    \label{fig:time_charts}
\end{figure}

\subsection{Real-world results}
\label{subsec:exp_real}

\textbf{Experimental setup: }
For the real-world experiments we used two unmodified Parrot Bebop 2 UAVs with an integrated electronic gimbal, a WiFi router and a standard desktop PC (Intel i7-8700 CPU and Nvidia GTX1060 GPU).
All communication between the drones and PC were handled via a ROS interface with the Bebop SKD. 
We transmitted images from the UAVs to the base station for the actor's visual detection and trajectory forecasting, and sent velocity commands back to the UAV after planning. 

% This offboard implementation was chosen due to computation restriction o the drone model used (Bebop2). Although, as validated in \cite{r1,r2,r3} , the decentralized pipeline is fully capable of running onboard in single board computers.

\textbf{E4) Flight among obstacle: } We tested the system by recording a moving actor with 2 drones in an environment with a virtual obstacle. 
Figure \ref{fig:study_case} depicts how the high-level central planner interacts with the local trajectory optimization method to calculate the final UAV paths. 
\textit{Drone 1} is optimized first, and takes a trajectory close to, but sufficiently far from the obstacle. 
\textit{Drone 2} is optimized next by the central planner. When it reaches the vicinity of the virtual obstacle, the planner brings its ideal path to a higher elevation, above the first drone's path, in order to avoid colliding with the obstacle while keeping the actor visible and avoiding visibility of \textit{drone 1}.
The central planner's output for drones 1 and 2 are colored in blue and red respectively.
The UAV's respective local planners receive the discrete high-level path and optimize it, creating a smooth trajectory output.
% During the maneuver, the 'drone 2' is able to keep thee actor in frame while avoiding to be seen by the other drone. 
After \textit{drone 2} reaches the left side of the actor, it switches to a slightly tilted and distant shot due to the shot diversity cost.

\textbf{E5) Dynamic actor: } We evaluated the system's capability to track and record an actor performing dynamic movements with abrupt motion changes, such as a person playing soccer. As seen in the supplementary video, both drones were able to safely keep the actor in frame through the entire test while exploring diverse viewpoints with low inter-drone visibility.

% We invite the reader to visualize our experiments in the supplementary video.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/study_case_4.png}
    \caption{\small Real-life flight among a simulated obstacle. On the left, the outputted sequence waypoints for each drone (red and blue) guide the locally optimized paths (yellow) towards a region free from obstacles and free of inter-drone visibility. Diverse shots can be seen during flight.
    \vspace{-2mm}}
    \label{fig:study_case}
\end{figure}
 
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/fut_red}
    \caption{\small Real-life flight following a highly dynamic actor playing soccer. The drones are able to keep up with abrupt motion motion changes while filming the actor.
    \vspace{-4mm}}
    \label{fig:fut}
\end{figure}
 



==> multidrone_icra2021 - Copy/inputs/4_exp_descriptors.tex <==
% !TEX root = ../root.tex


\subsection{Learning a Descriptor Space}
\label{subsec:exp_rep}



==> multidrone_icra2021 - Copy/inputs/4_exp_real.tex <==
% !TEX root = ../root.tex

\subsection{Real-World Results}
\label{subsec:exp_real}
\rbnote{to fill}
% \todo[inline]{experiment setup}
% \missingfigure{rviz img of the drone's path and actor's path}



jhbhjbjhbhjbjhbhjbjhbhjbjhbjhbjh
fdsfdsfs

dsfdsfdsf

2222222222222222
33333333333333333333

444444444444444

==> multidrone_icra2021 - Copy/inputs/4_exp_sim.tex <==
% !TEX root = ../root.tex

\subsection{Simulated navigation results}
\label{subsec:exp_sim}
\rbnote{to fill}

\missingfigure{rviz img of the drone's path and actor's path, with camera view image from each drone (2 cols)}
\rbnote{to fill}

==> multidrone_icra2021 - Copy/inputs/5_discussion.tex <==
% !TEX root = ../root.tex

\section{Conclusion and Discussion}
\label{sec:discussion}

In this paper we present a system for real-time coordination of aerial cameras for autonomous cinematography in dynamic and unscripted scenarios.
First, we formalize the multi-UAV filming problem in terms of its main objectives: maximizing shot diversity, avoiding inter-vehicle visibility and obeying high-level cinematographic guidelines.
Next, we develop a two-step approach for calculating the trajectory of each UAV, based on an efficient centralized greedy planner for viewpoint selection coupled with a decentralized trajectory optimizer to calculate smooth trajectories.
We validate our system in multiple simulated and real-world experiments, and show that it can successfully control a team of UAVs.
Additionally, we provide insights into how our methods can scale for larger numbers of UAVs in terms of planning time and memory. 

We note that the nature of trajectories generated with our system is highly dependent on the combination of relative weights between costs. 
Different applications may require distinct weighing schemes.
For instance, for a journalistic coverage the operator would likely increase the penalty on inter-drone visibility, while this weight could be negligible for footage generated in a 3D motion reconstruction application.

We are interested in extending this research in multiple future directions.
Despite using a decentralized trajectory optimization framework, our experiments in this paper were performed on a single desktop PC, and commands were then transmitted to each UAV individually in real time.
We are currently working on a new multi-UAV system with onboard processors, where one master drone will run the fast centralized planner and then communicate with all other UAVs via a mesh network so that each drone can optimize its own trajectories.
In addition, we plan to employ our system in novel applications such as 3D reconstruction of scenes in the wild. 
Even though multi-view systems are already well developed for indoors environments \cite{joo2015panoptic}, creating such systems for capturing images in natural environments is still an open research field.


==> multidrone_icra2021 - Copy/inputs/6_conclusion.tex <==
% !TEX root = ../root.tex

% \section{Conclusion}
% \label{sec:conclusion}

% We presented a framework to solve perception-control tasks that leverages readily available unsupervised real-world data together with simulated supervised training data.
% At the heart of our approach is a cross-modal Variational Auto-Encoder framework that jointly encodes sensor data and useful task-specific system state information. 
% The framework utilizes the variations introduced by the unsupervised real-world data and the task-specific information via the supervised simulated data and learn robust representations in an efficient manner. Simulation studies and real-world experiments highlight the effectiveness of the framework on the task of FPV drone racing. 

% Future work includes extension of the framework to other robotic tasks, consideration of multiple modalities beyond images and training via reinforcement learning methods. Additionally we are also exploring safety considerations in autonomy that combines the data-driven policies with formal methods based safety reasoning.

==> multidrone_icra2021 - Copy/macros/math_defns.tex <==

\newcommand{\Path}[1]{\xi_{#1}}
\newcommand{\cost}[0]{J}
\newcommand{\costFn}[1]{\cost \left( #1 \right)}

\newcommand{\costShot}[0]{\cost_\mathrm{shot}}
\newcommand{\costFnShot}[1]{\costShot \left( #1 \right)}

\newcommand{\costSmooth}[0]{\cost_\mathrm{smooth}}
\newcommand{\costFnSmooth}[1]{\costSmooth \left( #1 \right)}

\newcommand{\costOcc}[0]{\cost_\mathrm{occ}}
\newcommand{\costFnOcc}[1]{\costOcc \left( #1 \right)}

\newcommand{\costObs}[0]{\cost_\mathrm{obs}}
\newcommand{\costFnObs}[1]{\costObs \left( #1 \right)}

\newcommand{\costDiv}[0]{\cost_\mathrm{div}}
\newcommand{\costFnDiv}[1]{\costDiv \left( #1 \right)}

\newcommand{\costVis}[0]{\cost_\mathrm{vis}}
\newcommand{\costFnVis}[1]{\costVis \left( #1 \right)}

\newcommand{\costCine}[0]{\cost_\mathrm{cine}}
\newcommand{\costFnCine}[1]{\costCine \left( #1 \right)}

\newcommand{\map}[0]{\mathcal{M}}
\newcommand{\grid}[0]{\mathcal{G}}


==> multidrone_icra2021 - Copy/macros/math_operators.tex <==
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\diag}{diag}
\newcommand{\argmaxprob}[1]{\underset{#1}{\argmax}}
\newcommand{\argminprob}[1]{\underset{#1}{\argmin}}
\newcommand{\norm}[2]{\left|\left| #1 \right|\right|_{#2}}
\newcommand{\abs}[1]{\left|#1 \right|}
\newcommand{\card}[1]{\left|#1\right|}
\DeclareMathOperator*{\nullSpace}{Null}
\DeclareMathOperator*{\suchthat}{\;\; \mbox{s.t.} \;\;}
\newcommand{\expect}[2]{\mathbb{E}_{#1}\left[#2\right]}
% \newcommand{\prob}[1]{P\left(#1\right)}
\newcommand{\uniformSymb}[0]{\mathcal{U}}
\newcommand{\uniform}[1]{\uniformSymb\left(#1\right)}
\newcommand{\lebesgueSymb}[0]{\lambda}
\newcommand{\lebesgue}[1]{\lebesgueSymb\left(#1\right)}
\newcommand{\unitBall}[0]{\zeta_n}
\newcommand{\real}[0]{\mathbb{R}}
\newcommand{\positiveReal}[0]{\mathbb{R}_{\geq0}}
\newcommand{\domain}[1]{\mathbf{dom}\left(#1\right)}

\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}

\newcommand{\pair}[2]{\left( #1, #2\right)}
\newcommand{\set}[1]{\left\lbrace #1\right\rbrace}
\newcommand{\seq}[2]{\left(#1_{1}, #1_{2}, \ldots, #1_{#2}\right)}
\newcommand{\seqset}[2]{\left\lbrace#1_{1}, #1_{2}, \ldots, #1_{#2}\right\rbrace}
\newcommand{\setst}[2]{\left\lbrace #1\;\middle|\;#2\right\rbrace}

\newcommand{\setInsert}[0]{\xleftarrow{\scriptscriptstyle +}}
\newcommand{\setRemove}[0]{\xleftarrow{\scriptscriptstyle -}}

\newcommand{\Ind}[0]{\mathbb{I}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\Not}[1]{\overbar{#1}}

%%% runtime
\newcommand{\bigo}[1]{\mathcal{O}\left(#1\right)}

\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}


==> multidrone_icra2021 - Copy/macros/text_shortcuts.tex <==
\newcommand{\etal}[0]{et al.}

\newcommand{\bisect}[0]{\textsc{BiSECt}\xspace}
\newcommand{\direct}[0]{\textsc{DiRECt}\xspace}
\newcommand{\directONLY}[0]{\textsc{DiRECtonly}\xspace}

\newcommand{\ecsq}[0]{EC\textsuperscript{2}\xspace}
\newcommand{\algName}[0]{\textsc{BiSECt}\xspace}
\newcommand{\algFullName}[0]{Bernoulli Subregion Edge Cutting\xspace}


\newcommand{\algRandom}[0]{\textsc{Random}\xspace}
\newcommand{\algMaxTally}[0]{\textsc{MaxTally}\xspace}
\newcommand{\algSetCover}[0]{\textsc{SetCover}\xspace}
\newcommand{\algMVOI}[0]{\textsc{MVoI}\xspace}

\newcommand{\probBernDRD}[0]{Bern-DRD\xspace}
\newcommand{\probBernDRDFull}[0]{decision region determination with independent Bernoulli tests\xspace}

\newcommand{\algMaxProbReg}[0]{\textsc{MaxProbReg}\xspace}

\newcommand{\algLazySP}[0]{\textsc{LazySP}\xspace}
\newcommand{\algLazySPSet}[0]{\textsc{LazySPSet}\xspace}


